eThor: Practical and Provably Sound Static Analysis of Ethereum Smart Contracts

Ethereum has emerged as the most popular smart contract development platform, with hundreds of thousands of contracts stored on the blockchain and covering a variety of application scenarios, such as auctions, trading platforms, and so on. Given their financial nature, security vulnerabilities may lead to catastrophic consequences and, even worse, they can be hardly fixed as data stored on the blockchain, including the smart contract code itself, are immutable. An automated security analysis of these contracts is thus of utmost interest, but at the same time technically challenging for a variety of reasons, such as the specific transaction-oriented programming mechanisms, which feature a subtle semantics, and the fact that the blockchain data which the contract under analysis interacts with, including the code of callers and callees, are not statically known. In this work, we present eThor, the first sound and automated static analyzer for EVM bytecode, which is based on an abstraction of the EVM bytecode semantics based on Horn clauses. In particular, our static analysis supports reachability properties, which we show to be sufficient for capturing interesting security properties for smart contracts (e.g., single-entrancy) as well as contract-specific functional properties. Our analysis is proven sound against a complete semantics of EVM bytecode and an experimental large-scale evaluation on real-world contracts demonstrates that eThor is practical and outperforms the state-of-the-art static analyzers: specifically, eThor is the only one to provide soundness guarantees, terminates on 95% of a representative set of real-world contracts, and achieves an F-measure (which combines sensitivity and specificity) of 89%.

==> Makefile <==
# Makefile

PACKAGE=acmart

SAMPLES = main.tex 

PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

# %.pdf:  %.dtx   $(PACKAGE).cls
# 	pdflatex $<
# 	- bibtex $*
# 	pdflatex $<
# 	- makeindex -s gind.ist -o $*.ind $*.idx
# 	- makeindex -s gglo.ist -o $*.gls $*.glo
# 	pdflatex $<
# 	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
# 	do pdflatex $<; done

# %.cls:   %.ins %.dtx  
# 	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  main.pdf *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.fdb_latexmk *.fls *.synctex.gz *.xcp


==> change-report.tex <==
%List of changes
We will in the following overview the requested changes and how they were addressed.

\begin{enumerate}
\item
Properties different from reentrancy
\begin{enumerate}
\item 
Clarification of \ethor{}'s capability to express functional correctness properties and static assertion checking and of how the case study testifies the feasibility of checking them.

{\newforshepherd
We changed the motivation of~\autoref{subsec:reachability} to highlight that all reachability properties presented in this section are in the scope of \ethor{}. In addition we adapted the introduction to~\autoref{sec:eval} to illustrate how the different parts of the practical evaluation (case study, testing, large-scale evaluation) serve to demonstrate how \ethor{} can automatically show the properties discussed in~\autoref{subsec:reachability} in practice.
}
\item
  Extension of the case study on the \lstinline|SafeMath| library to include more functional correctness properties. More precisely, we will use \ethor{} to show that in case that the computations of the different functions do not over- or underflow 1) they can halt regularly producing the correct result 2) if halting regularly they can produce nothing but the correct result

{\newforshepherd
We extended the case study with the described properties and adapted the explanation in~\autoref{subsec:case-study} accordingly. The details of the extended case study are spelled out in~\autoref{app:security-properties}. In case that the paper gets accepted, we will make the extended version of the paper (containing the appendix) as well as our sources available online, so that the details on the extended case study will be publicly accessible.
}
\end{enumerate}
\item
Related work. We will clarify the following points:
\begin{enumerate}
\item
POPL 2017 paper
\begin{enumerate}
\item
The paper does not provide a static analysis method for checking effective callback-freeness, but only a dynamic one (indeed they show that the static detection of effective callback-freeness is undecidable).
\end{enumerate}
\item
Osiris
\begin{enumerate}
\item
Osiris does not aim for soundness
\item
Osiris targets a different class of bugs (which is not semantically characterized)
\end{enumerate}
\item
More thorough discussion of the limitations of the other tools (as far as space permits) and how they are addressed by eThor
\end{enumerate}

{\newforshepherd
We added~\autoref{sec:related-work} where we discuss the POPL paper~\cite{grossman2017online} and Osiris~\cite{torres2018osiris}. Additionally, we use this section to give a summary of the soundness flaws detected in other tools (as spelled out in~\autoref{app:soundness-issues}) and to attach a short discussion on how \ethor{} overcomes these issues (as it was suggested by reviewers A and B).
}
\item
Evaluation
\begin{enumerate}
\item
More precise discussion on the data set, emphasizing that it consists of real-world contracts

{\newforshepherd
Throughout~\autoref{sec:eval} we clarified that the used data set contains real-world contracts. In particular, we added in~\autoref{subsec:reentrancy-eval} the description of how the data set was originally obtained by~\cite{kalra2018zeus}.
}
\end{enumerate}
\item
Improving readability
\begin{enumerate}
\item
More detailed explanation of the single-entrancy property

{\newforshepherd
We added a corresponding explanation in~\autoref{subsec:props}.
}
\item
Clearer comparison with~\cite{GMS::POST18} and~\cite{GMS::CAV18}

{\newforshepherd
We checked that the parts of the paper using material from~\cite{GMS::POST18} and ~\cite{GMS::CAV18} are well-marked, and updated the explanation of~\autoref{def:callunreachability} to be more explicit about this. Also, we included a discussion of~\cite{GMS::CAV18} in the newly created~\autoref{sec:related-work}.
}
\item
More comprehensive introduction of Horn clauses

{\newforshepherd
We added an explaining sentence in the introduction of~\autoref{sec:stat}.
}
\item
More thorough explanation of the formal analysis definition (soundness statement, relation between alpha and delta, etc.)

{\newforshepherd
We rewrote large parts of~\autoref{subsec:analysis-definition} to clarify how the different components of the analysis specification work together. 
Additionally, we added a more detailed explanation for the soundness statement in~\autoref{subsec:soundness}.
}
\item
Revision of section 4 to focus on the utilization of HoRSt in the analysis design

{\newforshepherd
We added a new subsection in~\autoref{sec:horst} that discusses the utilization of \horst{} in the design of static analyzers and also illustrates this process graphically in~\autoref{fig:horst-design}. For saving space, we in turn shortened the subsequent subsection, also removing the figure showing an example for the different \hornc{} clause transformations.
}
\item
Fixing the minor remarks mentioned in the reviews

{\newforshepherd
We adapted ~\autoref{fig:grammar'} and ~\autoref{fig:pred-signature} following the remarks of the reviewers. Also, we reworked~\autoref{subsec:reentrancy-eval} to give a better motivation for the experimental setup and shortened the section by removing one of the figures on the comparative evaluation results for the different transformations.
}
\end{enumerate}
\end{enumerate}


==> horst-compiler.tex <==
%Horst compiler

\subsubsection{Constant folding}
After all parameters have been instantiated, we apply a constant folding to the intermediate representation.
This is especially useful to simplify expressions generated with sum expressions and expressions that make use of values gathered during preanalysis \TODOF{reference example above}.\TODOM{this whole paragraph is out of context and unclear}

After constant folding, trivially false rules are removed to keep the \texttt{smt-lib} output smaller.

\subsubsection{Value encoding}
Although \texttt{smt-lib} provides facilities for defining custom data types, our preliminary experiments showed that in the given use case translating custom types to primitive once improved performance. \TODOM{this motivation is very weak}

The translation from expression of a custom \horst{} type to a sequence of primitive types is a simple recursive procedure:
If a type has more than one constructor, we insert an integer\footnote{In the special case of two constructors, a boolean is used.} that serves as the discriminant.
Afterwards for each constructor, this procedure is repeated for all types accepted by the constructor, leaving primitive types unmodified and translating arrays of custom types to sequences of arrays of primitive types.

This translation is applied to custom types appearing in predicates, applications of constructors and (in)equalities between expressions of custom types (which are lifted on the sequences).
Match expressions are compiled to nested if-then-else expressions, containing equalities on discriminants in the condition and computations on the matched values in the branches.\TODOM{these last two paragraphs could be quickly summerized in one or two sentences, referring if you wish to the long version}


\paragraph{Implementation}
We strived for simplicity in our implementation, therefore every step in our compilation (inlining operations, translating \horst{} types to types of the underlying equational theory, instantiating the parameters, various optimizations) is implemented as a transformation of immutable data structures.

\paragraph{Pre-processing}
\begin{figure}[h!]
\includegraphics[width=\linewidth]{analysis_pic.pdf}
\caption{Analysis Outline.}
\label{fig:analysis-outline}
\end{figure}
The workflow outline of the static analysis tool for Ethereum smart contracts is depicted in \autoref{fig:analysis-outline}. The tool requires two kinds of inputs.
The first input is a Smart contract in the form of EVM bytecode which can be supplied in form of a \texttt{.txt} file or directly fetched from the blockchain using the EtherScan API~\cite{etherscan}. The second input is a (series of) files in $\horst$-format specifying the \hornc-clause based abstraction (parametrized by the contract to be analyzed) to be created.
After performing a constant analysis which we will describe in the next paragraph, optionally the low-level optimizations discussed in \autoref{subsec:ll-optimizations} are applied. Afterwards the $\horst$ compiler generates an \texttt{smt-lib} specification of the abstraction and the encoded queries.  Finally $\zz$ using one of its fixed point engines is invoked on the obtained file, determining the reachability for each of the present queries.

After processing the inputs we obtain an intermediate representation which can be directly supplied to our \hornc clause generation engine, or pre-processed by a Constant analysis.
\TODOC{This is not really true right? The constant analysis is performed on the smart contracts and not on the analysis specification}

 Our constant analysis is specific to the Ethereum platform. It boosts the overall performance of the tool as we identified during our experiments, mostly due to the fact that a number of arithmetic operations are very costly if performed by $\zz$ during the analysis, but can be easily precomputed by our constant analysis. The constant analysis also helps to identify jump targets and thereby to recover the contract's control flow graph (CFG).
In order for our constant analysis to be sound, we perform constant propagation only within atomic blocks, i.e., sequences of opcodes that contain control flow instructions such as $\JUMP$ in final position only.
The constant analysis results are used then later to reconstruct the CFG of a Smart contract. The CFG information is used to detect cycles, since for non-cyclic control flow graphs, we can re-run the constant analysis walking the nodes of the CFG in topological order thus enabling a better constant recovery.
\else



%%%% The following is a bit out of place (it's an addition for the testing)

The official test cases specify the execution and transaction environment in which a provided code snippet shall be executed and then specify pre- and postconditions on the global storage.
Using the ideas presented in \autoref{subsubsec:testing-formal}, we automatically generated soundness and precision tests from the official test cases as shown in \autoref{fig:tests}.

Given the expected storage configuration at the end of the execution (returned
by \texttt{postStorage}) and the last program counter of the analyzed test case (given by \texttt{lastPc}), the query \texttt{correctValues} checks if all the
specified storage values (or their over-approximation $\top$) are derivable. The second set of queries (implemented by \texttt{uniqueValues})
concerns precision: if we can only derive the required value, our derivation is
considered precise (if $\top$ or a wrong value is derived the test fails). The uniqueness test can be seen as a precision test as defined in \autoref{subsubsec:testing-formal} when assuming soundness (which excludes the derivability of incomparable values).

\lstset{escapechar=, language=HoRSt}
\begin{figure}[htb]
\begin{lstlisting}
    op abseq(a: AbsDom, b: AbsDom): bool :=
        match (a, b) with | (@V(x), @V(y)) => x = y
                          | _ => true;
    op absneq(a: AbsDom, b: AbsDom): bool :=
        match (a, b) with | (@V(x), @V(y)) => x != y
                          | _ => true;

    test correctValues expect SAT
        for (!pc: int) in lastPc()
        [?size: int, ?sa: array<AbsDom>,
         ?mem: array<AbsDom>, ?stor: array<AbsDom>, ?cd: int]
        for (!offset: int, !value: int) in postStorage():
            && abseq(select ?stor !offset,@V(!value)),
        MState{!pc}(?size, ?sa, ?mem, ?stor, ?cd);

    test uniqueValues expect UNSAT
        for (!pc: int) in lastPc()
        [?size: int, ?sa: array<AbsDom>,
         ?mem: array<AbsDom>, ?stor: array<AbsDom>, ?cd: int]
        for (!offset: int, !value: int) in postStorage():
            || absneq(select ?stor !offset,@V(!value)),
        MState{!pc}(?size, ?sa, ?mem, ?stor, ?cd);
\end{lstlisting}
\caption{\horst{}-tests for precision and soundness of the analysis.}
\label{fig:tests}
\end{figure}
Note that for specifying the soundness and precision tests, we make use of special instances of the iteration operator presented in \autoref{subsubsec:iteration} that implement the operators $\bigwedge_{i \in I}$ (\texttt{\&\&}) and $\bigvee_{i \in I}$ (\texttt{||}) .

==> stat-extended.tex <==
% extended material for analysis
\begin{figure*}[!t]
\begin{minipage}{.4\textwidth}
{\small
\begin{align*}
\abs{a} \absop{+} \abs{b} \define
\begin{cases}
\abs{a} + \abs{b} & \abs{a}, \abs{b} \in \NN \\
\top & \text{otherwise}
\end{cases}
\end{align*}}
\caption{Addition on abstract values.}
\label{fig:absadd}
\end{minipage}
%
\begin{minipage}{.59\textwidth}
{\small
\begin{align*}
\extractbyte{\abs{v}}{i}% 
&\define
\begin{cases}
\left \lfloor \frac{\abs{v}}{256^{31-i}} \right \rfloor \mod{256} & \abs{v} \in \NN ~\land~ i \in \{0, \dots 31 \}\\
\top & \text{otherwise}
\end{cases}
\end{align*}}
\caption{Byte extraction on an abstract value.}
\label{fig:absbyteextract}
\end{minipage}
\end{figure*}

\begin{figure*}[!t]
{\small
\begin{align*}
\updateit{i \in l}{f}{e_1(i)}{e_2(i)}
&\define
\begin{cases}
f & l = \nil \\
\updateit{i \in l'}{(\update{f}{e_1(x)}{e_2(x)})}{e_1(i)}{e_2(i)} & l = \cons{x}{l'}
\end{cases}
\end{align*}}
\caption{Iterative update operation on a function $f \in X \to Y$. The operator iterates over a list $l \in \listsof{Z}$ and updates the positions of $f$ defined by $e_1 \in Z \to X$ with values defined by $e_2 \in Z \to Y$. }
\label{fig:itmemupdate}
\end{figure*}
